Performance of novel VUV-sensitive Silicon Photo-Multipliers for nEXO

Liquid xenon time projection chambers are promising detectors to search for neutrinoless double beta decay (0$\nu \beta \beta$), due to their response uniformity, monolithic sensitive volume, scalability to large target masses, and suitability for extremely low background operations. The nEXO collaboration has designed a tonne-scale time projection chamber that aims to search for 0$\nu \beta \beta$ of \ce{^{136}Xe} with projected half-life sensitivity of $1.35\times 10^{28}$~yr. To reach this sensitivity, the design goal for nEXO is $\leq$1\% energy resolution at the decay $Q$-value ($2458.07\pm 0.31$~keV). Reaching this resolution requires the efficient collection of both the ionization and scintillation produced in the detector. The nEXO design employs Silicon Photo-Multipliers (SiPMs) to detect the vacuum ultra-violet, 175 nm scintillation light of liquid xenon. This paper reports on the characterization of the newest vacuum ultra-violet sensitive Fondazione Bruno Kessler VUVHD3 SiPMs specifically designed for nEXO, as well as new measurements on new test samples of previously characterised Hamamatsu VUV4 Multi Pixel Photon Counters (MPPCs). Various SiPM and MPPC parameters, such as dark noise, gain, direct crosstalk, correlated avalanches and photon detection efficiency were measured as a function of the applied over voltage and wavelength at liquid xenon temperature (163~K). The results from this study are used to provide updated estimates of the achievable energy resolution at the decay $Q$-value for the nEXO design.

==> SiPM characterisation for nEXO/authors_full.tex <==
\newcommand{\Stanford}{1}
\newcommand{\Erlangen}{2}
\newcommand{\Yale}{3}
\newcommand{\Bama}{4}
\newcommand{\Triumph}{5}
\newcommand{\Carleton}{6}
\newcommand{\Indiana}{7}
\newcommand{\PNL}{8}
\newcommand{\Duke}{9}
\newcommand{\Illinois}{10}
\newcommand{\ITEP}{11}
\newcommand{\Sherbrooke}{13}
\newcommand{\SD}{12}
\newcommand{\LLNL}{14}
\newcommand{\RPI}{15}
\newcommand{\McGill}{16}
\newcommand{\IHEP}{17}
\newcommand{\IME}{18}
\newcommand{\Colorado}{19}
\newcommand{\BNL}{20}
\newcommand{\Laurentian}{21}
\newcommand{\Wilmington}{22}
\newcommand{\SLAC}{23}
\newcommand{\Drexel}{24}
\newcommand{\ORNL}{25}
\newcommand{\UMass}{26}
\newcommand{\Stony}{27}
\newcommand{\IBS}{28}
\newcommand{\LHEP}{29}


\author[\Stanford,\Erlangen,\Yale]{A.~Jamil\IEEEauthorrefmark{1}\thanks{\IEEEauthorrefmark{1}Corresponding Author}}%
\author[\Erlangen]{T.~Ziegler}%
\author[\Erlangen]{P.~Hufschmidt}%
\author[\Stanford]{G.~Li}%
\author[\Stanford]{L.~Lupin-Jimenez}%
\author[\Erlangen]{T.~Michel}%
\author[\Bama]{I.~Ostrovskiy}%
\author[\Triumph]{F.~Reti\`ere}%
\author[\Erlangen]{J.~Schneider}%
\author[\Erlangen]{M.~Wagenpfeil}%
\author[\Carleton]{A.~Alamre}%
\author[\Indiana]{J.~B.~Albert}%
\author[\Erlangen]{G.~Anton}%
\author[\PNL]{I.~J.~Arnquist}%
\author[\Carleton]{I.~Badhrees\IEEEauthorrefmark{2}\thanks{\IEEEauthorrefmark{2}Home institute King Abdulaziz City for Science and Technology,\\ ${}$\hspace{20pt} KACST, Riyadh 11442, Saudi Arabia}}%
\author[\Duke]{P.~S.~Barbeau}%
\author[\Illinois]{D.~Beck}%
\author[\ITEP]{V.~Belov}%
\author[\SD]{T.~Bhatta}%
\author[\Sherbrooke]{F.~Bourque}%
\author[\LLNL]{J.~P.~Brodsky}%
\author[\RPI]{E.~Brown}%
\author[\McGill,\Triumph]{T.~Brunner}%
\author[\ITEP]{A.~Burenkov}%
\author[\IHEP]{G.~F.~Cao\IEEEauthorrefmark{3}\thanks{\IEEEauthorrefmark{3}also at University of Chinese Academy of Sciences, \\ ${}$\hspace{22pt}Beijing 100049, China}}%
\author[\IME]{L.~Cao}%
\author[\IHEP]{W.~R.~Cen}%
\author[\Colorado]{C.~Chambers}%
\author[\Sherbrooke]{S.~A.~Charlebois}%
\author[\BNL]{M.~Chiu}%
\author[\Laurentian]{B.~Cleveland\IEEEauthorrefmark{4}\thanks{\IEEEauthorrefmark{4}also at SNOLAB, Ontario, Canada}}%
\author[\Illinois]{M.~Coon}%
\author[\Sherbrooke]{M.~C{\^o}t{\'e}}%
\author[\Colorado]{A.~Craycraft}%
\author[\Carleton]{W.~Cree}%
\author[\Stanford]{J.~Dalmasson}%
\author[\Wilmington]{T.~Daniels}%
\author[\McGill]{L.~Darroch}%
\author[\Indiana]{S.~J.~Daugherty}%
\author[\SD]{J.~Daughhetee}%
\author[\SLAC]{S.~Delaquis\IEEEauthorrefmark{5}\thanks{\IEEEauthorrefmark{5}deceased}}%
\author[\Laurentian]{A.~Der~Mesrobian-Kabakian}%
\author[\Stanford]{R.~DeVoe}%
\author[\Triumph]{J.~Dilling}%
\author[\IHEP]{Y.~Y.~Ding}%
\author[\Drexel]{M.~J.~Dolinski}%
\author[\SLAC]{A.~Dragone}%
\author[\Illinois]{J.~Echevers}%
\author[\ORNL]{L.~Fabris}%
\author[\Colorado]{D.~Fairbank}%
\author[\Colorado]{W.~Fairbank}%
\author[\Laurentian]{J.~Farine}%
\author[\UMass]{S.~Feyzbakhsh}%
\author[\Sherbrooke]{R.~Fontaine}%
\author[\Stanford]{D.~Fudenberg}%
\author[\Triumph]{G.~Gallina}%
\author[\BNL]{G.~Giacomini}%
\author[\Carleton,\Triumph]{R.~Gornea}%
\author[\Stanford]{G.~Gratta}%
\author[\Drexel]{E.~V.~Hansen}%
\author[\Colorado]{D.~Harris}%
\author[\SD]{M.~Hasan}%
\author[\LLNL]{M.~Heffner}%
\author[\Erlangen]{J.~H{\"o}{\ss}l}%
\author[\PNL]{E.~W.~Hoppe}%
\author[\LLNL]{A.~House}%
\author[\Bama]{M.~Hughes}%
\author[\McGill]{Y.~Ito}%
\author[\Colorado]{A.~Iverson}%
\author[\Carleton]{C.~Jessiman}%
\author[\Stanford]{M.~J.~Jewell}%
\author[\IHEP]{X.~S.~Jiang}%
\author[\ITEP]{A.~Karelin}%
\author[\Indiana,\SLAC]{L.~J.~Kaufman}%
\author[\Carleton]{T.~Koffas}%
\author[\Stanford]{S.~Kravitz\IEEEauthorrefmark{6}\thanks{\IEEEauthorrefmark{6}now at Lawrence Berkeley National Lab}}%
\author[\Triumph]{R.~Kr\"ucken}%
\author[\ITEP]{A.~Kuchenkov}%
\author[\Stony]{K.~S.~Kumar}%
\author[\Triumph]{Y.~Lan}%
\author[\SD]{A.~Larson}%
\author[\IBS]{D.~S.~Leonard}%
\author[\Illinois]{S.~Li}%
\author[\Yale]{Z.~Li}%
\author[\Laurentian]{C.~Licciardi}%
\author[\Drexel]{Y.~H.~Lin}%
\author[\IHEP]{P.~Lv}%
\author[\SD]{R.~MacLellan}%
\author[\SLAC]{B.~Mong}%
\author[\Yale]{D.~C.~Moore}%
\author[\McGill]{K.~Murray}%
\author[\ORNL]{R.~J.~Newby}%
\author[\IHEP]{Z.~Ning}%
\author[\Stony]{O.~Njoya}%
\author[\Sherbrooke]{F.~Nolet}%
\author[\Bama]{O.~Nusair}%
\author[\RPI]{K.~Odgers}%
\author[\SLAC]{A.~Odian}%
\author[\SLAC]{M.~Oriunno}%
\author[\PNL]{J.~L.~Orrell}%
\author[\PNL]{G.~S.~Ortega}%
\author[\PNL]{C.~T.~Overman}%
\author[\Sherbrooke]{S.~Parent}%
\author[\Bama]{A.~Piepke}%
\author[\UMass]{A.~Pocar}%
\author[\Sherbrooke]{J.-F.~Pratte}%
\author[\IME]{D.~Qiu}%
\author[\BNL]{V.~Radeka}%
\author[\BNL]{E.~Raguzin}%
\author[\BNL]{T.~Rao}%
\author[\BNL]{S.~Rescia}%
\author[\Laurentian]{A.~Robinson}%
\author[\Sherbrooke]{T.~Rossignol}%
\author[\SLAC]{P.~C.~Rowson}%
\author[\Sherbrooke]{N.~Roy}%
\author[\PNL]{R.~Saldanha}%
\author[\LLNL]{S.~Sangiorgio}%
\author[\Erlangen]{S.~Schmidt}%
\author[\Stanford]{A.~Schubert\IEEEauthorrefmark{7}\thanks{\IEEEauthorrefmark{7}now at OneBridge Solutions, Boise, ID}}
\author[\Carleton]{D.~Sinclair}%
\author[\SLAC]{K.~Skarpaas VIII}%
\author[\Bama]{A.~K.~Soma}%
\author[\Sherbrooke]{G.~St-Hilaire}%
\author[\ITEP]{V.~Stekhanov}%
\author[\LLNL]{T.~Stiegler}%
\author[\IHEP]{X.~L.~Sun}%
\author[\Stony]{M.~Tarka\IEEEauthorrefmark{8}\thanks{\IEEEauthorrefmark{8}now at University of Massachusetts, Amherst}}%
\author[\Colorado]{J.~Todd}%
\author[\IHEP]{T.~Tolba}%
\author[\McGill]{T.~I.~Totev}%
\author[\PNL]{R.~Tsang}%
\author[\BNL]{T.~Tsang}%
\author[\Sherbrooke]{F.~Vachon}%
\author[\Carleton]{B.~Veenstra}%
\author[\Bama]{V.~Veeraraghavan}%
\author[\Indiana]{G.~Visser}%
\author[\LHEP]{J.-L.~Vuilleumier}%
\author[\IME]{Q.~Wang}%
\author[\Carleton]{J.~Watkins}%
\author[\Stanford]{M.~Weber}%
\author[\IHEP]{W.~Wei}%
\author[\IHEP]{L.~J.~Wen}%
\author[\Laurentian]{U.~Wichoski}%
\author[\Erlangen]{G.~Wrede}%
\author[\Stanford]{S.~X.~Wu}%
\author[\IHEP]{W.~H.~Wu}%
\author[\Yale]{Q.~Xia}%
\author[\Illinois]{L.~Yang}%
\author[\Drexel]{Y.-R.~Yen}%
\author[\ITEP]{O.~Zeldovich}%
\author[\IHEP]{X.~Zhang\IEEEauthorrefmark{9}\thanks{\IEEEauthorrefmark{9}now at Tsinghua University, Beijing, China}}%
\author[\IHEP]{J.~Zhao}%
\author[\IME]{Y.~Zhou}%


\affil[\Stanford]{Physics Department, Stanford University, Stanford, California 94305, USA}
\affil[\Erlangen]{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander University Erlangen-N\"urnberg, Erlangen 91058, Germany}
\affil[\Yale]{Department of Physics, Yale University, New Haven, CT 06511, USA}
\affil[\Bama]{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\affil[\Triumph]{TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\affil[\Carleton]{Department of Physics, Carleton University, Ottawa, Ontario K1S 5B6, Canada}
\affil[\Indiana]{Department of Physics and CEEM, Indiana University, Bloomington, IN 47405, USA}
\affil[\PNL]{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\affil[\Duke]{Department of Physics, Duke University, and Triangle Universities Nuclear Laboratory (TUNL), Durham, NC 27708, USA}
\affil[\Illinois]{Physics Department, University of Illinois, Urbana-Champaign, IL 61801, USA}
\affil[\ITEP]{Institute for Theoretical and Experimental Physics named by A.~I.~Alikhanov of National Research Center "Kurchatov Institute", Moscow 117218, Russia}
\affil[\SD]{Department of Physics, University of South Dakota, Vermillion, SD 57069, USA}
\affil[\Sherbrooke]{Universit\'e de Sherbrooke, Sherbrooke, Qu{\'e}bec J1K 2R1, Canada}
\affil[\LLNL]{Lawrence Livermore National Laboratory, Livermore, CA 94550, USA}
\affil[\RPI]{Department of Physics, Applied Physics and Astronomy, Rensselaer Polytechnic Institute, Troy, NY 12180, USA}
\affil[\McGill]{Physics Department, McGill University, Montr{\'e}al, Qu{\'e}bec H3A 2T8, Canada}
\affil[\IHEP]{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\affil[\IME]{Institute of Microelectronics, Chinese Academy of Sciences, Beijing 100029, China}
\affil[\Colorado]{Physics Department, Colorado State University, Fort Collins, CO 80523, USA}
\affil[\BNL]{Brookhaven National Laboratory, Upton, NY 11973, USA}
\affil[\Laurentian]{Department of Physics, Laurentian University, Sudbury, Ontario P3E 2C6, Canada}
\affil[\Wilmington]{Department of Physics and Physical Oceanography, University of North Carolina at Wilmington, Wilmington, NC 28403, USA}
\affil[\SLAC]{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\affil[\Drexel]{Department of Physics, Drexel University, Philadelphia, PA 19104, USA}
\affil[\ORNL]{Oak Ridge National Laboratory, Oak Ridge, TN 37831, USA}
\affil[\UMass]{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\affil[\Stony]{Department of Physics and Astronomy, Stony Brook University, SUNY, Stony Brook, NY 11794, USA}
\affil[\IBS]{IBS Center for Underground Physics, Daejeon 34126, Korea}
\affil[\LHEP]{LHEP, Albert Einstein Center, University of Bern, Bern CH-3012, Switzerland}











==> authors_full.tex <==
\newcommand{\Stanford}{1}
\newcommand{\Erlangen}{2}
\newcommand{\Yale}{3}
\newcommand{\Bama}{4}
\newcommand{\Triumph}{5}
\newcommand{\Carleton}{6}
\newcommand{\Indiana}{7}
\newcommand{\PNL}{8}
\newcommand{\Duke}{9}
\newcommand{\Illinois}{10}
\newcommand{\ITEP}{11}
\newcommand{\Sherbrooke}{13}
\newcommand{\SD}{12}
\newcommand{\LLNL}{14}
\newcommand{\RPI}{15}
\newcommand{\McGill}{16}
\newcommand{\IHEP}{17}
\newcommand{\IME}{18}
\newcommand{\Colorado}{19}
\newcommand{\BNL}{20}
\newcommand{\Laurentian}{21}
\newcommand{\Wilmington}{22}
\newcommand{\SLAC}{23}
\newcommand{\Drexel}{24}
\newcommand{\ORNL}{25}
\newcommand{\UMass}{26}
\newcommand{\Stony}{27}
\newcommand{\IBS}{28}
\newcommand{\LHEP}{29}


\author[\Stanford,\Erlangen,\Yale]{A.~Jamil\IEEEauthorrefmark{1}\thanks{\IEEEauthorrefmark{1}Corresponding Author}}%
\author[\Erlangen]{T.~Ziegler}%
\author[\Erlangen]{P.~Hufschmidt}%
\author[\Stanford]{G.~Li}%
\author[\Stanford]{L.~Lupin-Jimenez}%
\author[\Erlangen]{T.~Michel}%
\author[\Bama]{I.~Ostrovskiy}%
\author[\Triumph]{F.~Reti\`ere}%
\author[\Erlangen]{J.~Schneider}%
\author[\Erlangen]{M.~Wagenpfeil}%
\author[\Carleton]{A.~Alamre}%
\author[\Indiana]{J.~B.~Albert}%
\author[\Erlangen]{G.~Anton}%
\author[\PNL]{I.~J.~Arnquist}%
\author[\Carleton]{I.~Badhrees\IEEEauthorrefmark{2}\thanks{\IEEEauthorrefmark{2}Home institute King Abdulaziz City for Science and Technology,\\ ${}$\hspace{20pt} KACST, Riyadh 11442, Saudi Arabia}}%
\author[\Duke]{P.~S.~Barbeau}%
\author[\Illinois]{D.~Beck}%
\author[\ITEP]{V.~Belov}%
\author[\SD]{T.~Bhatta}%
\author[\Sherbrooke]{F.~Bourque}%
\author[\LLNL]{J.~P.~Brodsky}%
\author[\RPI]{E.~Brown}%
\author[\McGill,\Triumph]{T.~Brunner}%
\author[\ITEP]{A.~Burenkov}%
\author[\IHEP]{G.~F.~Cao\IEEEauthorrefmark{3}\thanks{\IEEEauthorrefmark{3}also at University of Chinese Academy of Sciences, \\ ${}$\hspace{22pt}Beijing 100049, China}}%
\author[\IME]{L.~Cao}%
\author[\IHEP]{W.~R.~Cen}%
\author[\Colorado]{C.~Chambers}%
\author[\Sherbrooke]{S.~A.~Charlebois}%
\author[\BNL]{M.~Chiu}%
\author[\Laurentian]{B.~Cleveland\IEEEauthorrefmark{4}\thanks{\IEEEauthorrefmark{4}also at SNOLAB, Ontario, Canada}}%
\author[\Illinois]{M.~Coon}%
\author[\Sherbrooke]{M.~C{\^o}t{\'e}}%
\author[\Colorado]{A.~Craycraft}%
\author[\Carleton]{W.~Cree}%
\author[\Stanford]{J.~Dalmasson}%
\author[\Wilmington]{T.~Daniels}%
\author[\McGill]{L.~Darroch}%
\author[\Indiana]{S.~J.~Daugherty}%
\author[\SD]{J.~Daughhetee}%
\author[\SLAC]{S.~Delaquis\IEEEauthorrefmark{5}\thanks{\IEEEauthorrefmark{5}deceased}}%
\author[\Laurentian]{A.~Der~Mesrobian-Kabakian}%
\author[\Stanford]{R.~DeVoe}%
\author[\Triumph]{J.~Dilling}%
\author[\IHEP]{Y.~Y.~Ding}%
\author[\Drexel]{M.~J.~Dolinski}%
\author[\SLAC]{A.~Dragone}%
\author[\Illinois]{J.~Echevers}%
\author[\ORNL]{L.~Fabris}%
\author[\Colorado]{D.~Fairbank}%
\author[\Colorado]{W.~Fairbank}%
\author[\Laurentian]{J.~Farine}%
\author[\UMass]{S.~Feyzbakhsh}%
\author[\Sherbrooke]{R.~Fontaine}%
\author[\Stanford]{D.~Fudenberg}%
\author[\Triumph]{G.~Gallina}%
\author[\BNL]{G.~Giacomini}%
\author[\Carleton,\Triumph]{R.~Gornea}%
\author[\Stanford]{G.~Gratta}%
\author[\Drexel]{E.~V.~Hansen}%
\author[\Colorado]{D.~Harris}%
\author[\SD]{M.~Hasan}%
\author[\LLNL]{M.~Heffner}%
\author[\Erlangen]{J.~H{\"o}{\ss}l}%
\author[\PNL]{E.~W.~Hoppe}%
\author[\LLNL]{A.~House}%
\author[\Bama]{M.~Hughes}%
\author[\McGill]{Y.~Ito}%
\author[\Colorado]{A.~Iverson}%
\author[\Carleton]{C.~Jessiman}%
\author[\Stanford]{M.~J.~Jewell}%
\author[\IHEP]{X.~S.~Jiang}%
\author[\ITEP]{A.~Karelin}%
\author[\Indiana,\SLAC]{L.~J.~Kaufman}%
\author[\Carleton]{T.~Koffas}%
\author[\Stanford]{S.~Kravitz\IEEEauthorrefmark{6}\thanks{\IEEEauthorrefmark{6}now at Lawrence Berkeley National Lab}}%
\author[\Triumph]{R.~Kr\"ucken}%
\author[\ITEP]{A.~Kuchenkov}%
\author[\Stony]{K.~S.~Kumar}%
\author[\Triumph]{Y.~Lan}%
\author[\SD]{A.~Larson}%
\author[\IBS]{D.~S.~Leonard}%
\author[\Illinois]{S.~Li}%
\author[\Yale]{Z.~Li}%
\author[\Laurentian]{C.~Licciardi}%
\author[\Drexel]{Y.~H.~Lin}%
\author[\IHEP]{P.~Lv}%
\author[\SD]{R.~MacLellan}%
\author[\SLAC]{B.~Mong}%
\author[\Yale]{D.~C.~Moore}%
\author[\McGill]{K.~Murray}%
\author[\ORNL]{R.~J.~Newby}%
\author[\IHEP]{Z.~Ning}%
\author[\Stony]{O.~Njoya}%
\author[\Sherbrooke]{F.~Nolet}%
\author[\Bama]{O.~Nusair}%
\author[\RPI]{K.~Odgers}%
\author[\SLAC]{A.~Odian}%
\author[\SLAC]{M.~Oriunno}%
\author[\PNL]{J.~L.~Orrell}%
\author[\PNL]{G.~S.~Ortega}%
\author[\PNL]{C.~T.~Overman}%
\author[\Sherbrooke]{S.~Parent}%
\author[\Bama]{A.~Piepke}%
\author[\UMass]{A.~Pocar}%
\author[\Sherbrooke]{J.-F.~Pratte}%
\author[\IME]{D.~Qiu}%
\author[\BNL]{V.~Radeka}%
\author[\BNL]{E.~Raguzin}%
\author[\BNL]{T.~Rao}%
\author[\BNL]{S.~Rescia}%
\author[\Laurentian]{A.~Robinson}%
\author[\Sherbrooke]{T.~Rossignol}%
\author[\SLAC]{P.~C.~Rowson}%
\author[\Sherbrooke]{N.~Roy}%
\author[\PNL]{R.~Saldanha}%
\author[\LLNL]{S.~Sangiorgio}%
\author[\Erlangen]{S.~Schmidt}%
\author[\Stanford]{A.~Schubert\IEEEauthorrefmark{7}\thanks{\IEEEauthorrefmark{7}now at OneBridge Solutions, Boise, ID}}
\author[\Carleton]{D.~Sinclair}%
\author[\SLAC]{K.~Skarpaas VIII}%
\author[\Bama]{A.~K.~Soma}%
\author[\Sherbrooke]{G.~St-Hilaire}%
\author[\ITEP]{V.~Stekhanov}%
\author[\LLNL]{T.~Stiegler}%
\author[\IHEP]{X.~L.~Sun}%
\author[\Stony]{M.~Tarka\IEEEauthorrefmark{8}\thanks{\IEEEauthorrefmark{8}now at University of Massachusetts, Amherst}}%
\author[\Colorado]{J.~Todd}%
\author[\IHEP]{T.~Tolba}%
\author[\McGill]{T.~I.~Totev}%
\author[\PNL]{R.~Tsang}%
\author[\BNL]{T.~Tsang}%
\author[\Sherbrooke]{F.~Vachon}%
\author[\Carleton]{B.~Veenstra}%
\author[\Bama]{V.~Veeraraghavan}%
\author[\Indiana]{G.~Visser}%
\author[\LHEP]{J.-L.~Vuilleumier}%
\author[\IME]{Q.~Wang}%
\author[\Carleton]{J.~Watkins}%
\author[\Stanford]{M.~Weber}%
\author[\IHEP]{W.~Wei}%
\author[\IHEP]{L.~J.~Wen}%
\author[\Laurentian]{U.~Wichoski}%
\author[\Erlangen]{G.~Wrede}%
\author[\Stanford]{S.~X.~Wu}%
\author[\IHEP]{W.~H.~Wu}%
\author[\Yale]{Q.~Xia}%
\author[\Illinois]{L.~Yang}%
\author[\Drexel]{Y.-R.~Yen}%
\author[\ITEP]{O.~Zeldovich}%
\author[\IHEP]{X.~Zhang\IEEEauthorrefmark{9}\thanks{\IEEEauthorrefmark{9}now at Tsinghua University, Beijing, China}}%
\author[\IHEP]{J.~Zhao}%
\author[\IME]{Y.~Zhou}%


\affil[\Stanford]{Physics Department, Stanford University, Stanford, California 94305, USA}
\affil[\Erlangen]{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander University Erlangen-N\"urnberg, Erlangen 91058, Germany}
\affil[\Yale]{Department of Physics, Yale University, New Haven, CT 06511, USA}
\affil[\Bama]{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\affil[\Triumph]{TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\affil[\Carleton]{Department of Physics, Carleton University, Ottawa, Ontario K1S 5B6, Canada}
\affil[\Indiana]{Department of Physics and CEEM, Indiana University, Bloomington, IN 47405, USA}
\affil[\PNL]{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\affil[\Duke]{Department of Physics, Duke University, and Triangle Universities Nuclear Laboratory (TUNL), Durham, NC 27708, USA}
\affil[\Illinois]{Physics Department, University of Illinois, Urbana-Champaign, IL 61801, USA}
\affil[\ITEP]{Institute for Theoretical and Experimental Physics named by A.~I.~Alikhanov of National Research Center "Kurchatov Institute", Moscow 117218, Russia}
\affil[\SD]{Department of Physics, University of South Dakota, Vermillion, SD 57069, USA}
\affil[\Sherbrooke]{Universit\'e de Sherbrooke, Sherbrooke, Qu{\'e}bec J1K 2R1, Canada}
\affil[\LLNL]{Lawrence Livermore National Laboratory, Livermore, CA 94550, USA}
\affil[\RPI]{Department of Physics, Applied Physics and Astronomy, Rensselaer Polytechnic Institute, Troy, NY 12180, USA}
\affil[\McGill]{Physics Department, McGill University, Montr{\'e}al, Qu{\'e}bec H3A 2T8, Canada}
\affil[\IHEP]{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\affil[\IME]{Institute of Microelectronics, Chinese Academy of Sciences, Beijing 100029, China}
\affil[\Colorado]{Physics Department, Colorado State University, Fort Collins, CO 80523, USA}
\affil[\BNL]{Brookhaven National Laboratory, Upton, NY 11973, USA}
\affil[\Laurentian]{Department of Physics, Laurentian University, Sudbury, Ontario P3E 2C6, Canada}
\affil[\Wilmington]{Department of Physics and Physical Oceanography, University of North Carolina at Wilmington, Wilmington, NC 28403, USA}
\affil[\SLAC]{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\affil[\Drexel]{Department of Physics, Drexel University, Philadelphia, PA 19104, USA}
\affil[\ORNL]{Oak Ridge National Laboratory, Oak Ridge, TN 37831, USA}
\affil[\UMass]{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\affil[\Stony]{Department of Physics and Astronomy, Stony Brook University, SUNY, Stony Brook, NY 11794, USA}
\affil[\IBS]{IBS Center for Underground Physics, Daejeon 34126, Korea}
\affil[\LHEP]{LHEP, Albert Einstein Center, University of Bern, Bern CH-3012, Switzerland}










